Robust and Efficient Depth-based Obstacle Avoidance for Autonomous Miniaturized UAVs

Nano-size drones hold enormous potential to explore unknown and complex environments. Their small size makes them agile and safe for operation close to humans and allows them to navigate through narrow spaces. However, their tiny size and payload restrict the possibilities for on-board computation and sensing, making fully autonomous flight extremely challenging. The first step towards full autonomy is reliable obstacle avoidance, which has proven to be technically challenging by itself in a generic indoor environment. Current approaches utilize vision-based or 1-dimensional sensors to support nano-drone perception algorithms. This work presents a lightweight obstacle avoidance system based on a novel millimeter form factor 64 pixels multi-zone Time-of-Flight (ToF) sensor and a generalized model-free control policy. Reported in-field tests are based on the Crazyflie 2.1, extended by a custom multi-zone ToF deck, featuring a total flight mass of 35g. The algorithm only uses 0.3% of the on-board processing power (210uS execution time) with a frame rate of 15fps, providing an excellent foundation for many future applications. Less than 10% of the total drone power is needed to operate the proposed perception system, including both lifting and operating the sensor. The presented autonomous nano-size drone reaches 100% reliability at 0.5m/s in a generic and previously unexplored indoor environment. The proposed system is released open-source with an extensive dataset including ToF and gray-scale camera data, coupled with UAV position ground truth from motion capture.

==> sources/table.tex <==
\begin{table*}
\begin{center}
\caption{Dataset description: multi-zone ToF sensor combined with the Vicon system, grayscale camera and the internal state estimator.}
\label{tab:pipe}
\begin{tabular}{ c  l  c  c  c  }
\hline
\hline
Test Reference & Description & Vicon & Camera & Test time [s]\\
\hline
\multicolumn{5}{c}{Linear movements in one direction} \\
\hline
A0  & Approach to an object with speed 0.75 m/s, then stop and get back with same speed                     & \checkmark & \checkmark & 22 \\
A1  & Approach to an object with speed 0.5 m/s untill crashes to object                                     & \checkmark & \checkmark & 2.6\\
A2  & Approach to an object with speed 0.5 m/s, then stop and get back with same speed                      & \checkmark & \checkmark & 21 \\
A3  & Approach to an object with speed 0.75 m/s, then stop and 360 rotate and get back                      & \checkmark & \checkmark & 25 \\
A4  & Approach to an object with speed 0.75 m/s, then stop and land in back                                 & \checkmark & \checkmark & 19 \\
A5  & Approach to an object with speed 1 m/s, then stop and get back with same speed                        & \checkmark & \checkmark & 33 \\
A6  & Approach to an object with speed 1 m/s, then stop and get back with same speed                        & \checkmark & \checkmark & 24 \\
A7  & Approach to an object with speed 1 m/s, then stop and get back with same speed                        & \checkmark & \checkmark & 30 \\
A8  & Approach not in straight way to object,stop and get back with angle                                   & \checkmark & \checkmark & 21 \\
A9 & Approach to an object with speed .75 m/s, then stop and get back with same speed                       & \checkmark & \checkmark & 19 \\
\hline
\multicolumn{5}{c}{Yaw Rotations} \\
\hline
R0  & Rotate close to the object with yaw rate of 50 degree/sec                                             & \checkmark & \checkmark & 42 \\
R1  & Rotate close to the object with yaw rate of 70 degree/sec                                             & \checkmark & \checkmark & 28 \\
R2  & Rotate close to the object with yaw rate of 90 degree/sec                                             & \checkmark & \checkmark & 24 \\
\hline
\multicolumn{5}{c}{Obstacle avoidance with fixed and moving objects} \\
\hline
O0  & Take off, Approach to hole, Land                                                                      & \checkmark & \checkmark & 26 \\
O1  & Take off, avoid obstacle, Land                                                                        & $\times$   & \checkmark & 23 \\
O2  & Take off, Rotate to left, Approach to chair                                                           & \checkmark & \checkmark & 15 \\
O3  & Take off, Approach to chair, Cross the chair, Land                                                    & \checkmark & \checkmark & 29 \\
O4  & Take off, Rotate to left, Avoid the chair, Move to its initial position, Land                         & \checkmark & \checkmark & 35 \\
O5  & Take off, Approach to chair, Cross the chair, Approach to wall, Land                                  & \checkmark & \checkmark & 7.3 \\
O6  & Take off, Rotate to left, Approach to chair, Cross the chair, Land                                    & \checkmark & \checkmark & 58 \\
O7  & Random Movement, rotate and scan in corridor                                                          & \checkmark & \checkmark & 42 \\
O8  & Take off, Approach to hole, Cross the hole, Land                                                      & \checkmark & \checkmark & 11 \\
O9 & Approach to hole, Cross the hole, Land                                                                 & $\times$   & \checkmark & 32 \\
%
O10  & Take off, Approach to hole, Cross the hole, Land                                                     & $\times$   & \checkmark & 24 \\
O11  & Take off, Approach to hole, Cross the hole, Land                                                     & $\times$   & \checkmark & 32 \\
O12  & Take off, Approach to door, Approach to hole, Cross the hole, Rotate to left, Land                   & $\times$   & \checkmark & 48 \\
O13  & Take off, Approach to door, Approach to hole, Cross the hole, Approach to table                      & $\times$   & \checkmark & 61 \\
O14  & Take off, altitude increase with object in front                                                     & $\times$   & \checkmark & 19 \\
O15  & Take off, altitude increase with object in front                                                     & $\times$   & \checkmark & 53 \\
O16  & Random human movement with different angles and different approaches                                 & \checkmark & \checkmark & 65 \\
O17  & Take off, Random human movement in front of drone, Land                                              & \checkmark & \checkmark & 97 \\
O18  & Take off, Move towards multiple walls between chairs, Land                                           & \checkmark & \checkmark & 21 \\
O19 & Lateral movements in front of two objects                                                             & $\times$   & \checkmark & 19 \\
%
O20  & Cross an hole between two objects                                                                    & $\times$   & \checkmark & 22 \\
O21  & Avoid an angled obstacle                                                                             & $\times$   & \checkmark & 11 \\
O22  & Take off, Approach to surface, Cross object, Move forward, Land                                      & \checkmark & \checkmark & 18 \\
O23  & Take off, Approach to chair, Approach to box, Rotate right, Move forward between 2 objects     
                                                                                                            & \checkmark & \checkmark & 35 \\
O24  & Take off, Cross obejcts, Land                                                                        & \checkmark & \checkmark & 16 \\
O25  & Take off, Approach to first object, rotate left, Move forward, Land                                  & $\times$   & \checkmark & 26 \\
O26  & Take off, Approach to first object, Approach to wall, Cross it by rotating to left, Land             & $\times$   & \checkmark & 37 \\
O27  & Take off, first object, Approach to 2nd object, Cross it by increasing the altitude, Land            & $\times$   & \checkmark & 40 \\
O28  & Take off, first object, Approach to 2nd object, Cross it by rotating to left                         & $\times$   & \checkmark & 43 \\
O29 & Take off, Land                                                                                        & $\times$   & \checkmark & 86 \\
\hline
\hline 
\end{tabular}
\end{center}
\end{table*}
